Decentralized Multi-Task Stochastic Optimization With Compressed Communications

We consider a multi-agent network where each node has a stochastic (local) cost function that depends on the decision variable of that node and a random variable, and further the decision variables of neighboring nodes are pairwise constrained. There is an aggregate objective function for the network, composed additively of the expected values of the local cost functions at the nodes, and the overall goal of the network is to obtain the minimizing solution to this aggregate objective function subject to all the pairwise constraints. This is to be achieved at the node level using decentralized information and local computation, with exchanges of only compressed information allowed by neighboring nodes. The paper develops algorithms and obtains performance bounds for two different models of local information availability at the nodes: (i) sample feedback, where each node has direct access to samples of the local random variable to evaluate its local cost, and (ii) bandit feedback, where samples of the random variables are not available, but only the values of the local cost functions at two random points close to the decision are available to each node. For both models, with compressed communication between neighbors, we have developed decentralized saddle-point algorithms that deliver performances no different (in order sense) from those without communication compression; specifically, we show that deviation from the global minimum value and violations of the constraints are upper-bounded by $\mathcal{O}(T^{-\frac{1}{2}})$ and $\mathcal{O}(T^{-\frac{1}{4}})$, respectively, where $T$ is the number of iterations. Numerical examples provided in the paper corroborate these bounds and demonstrate the communication efficiency of the proposed method.

==> algo_personalized.tex <==
In this section, we discuss our training algorithm `QuPeL' (stated in Algorithm \ref{algo:personalized}) for learning quantized personalized models for inference in context of federated learning. QuPeL builds up on the quantized training scheme presented in Section \ref{sec:centralized} by learning a set of model parameters $\{\bx_i\}_{i=1}^{n}$ and quantization vectors (centers) $\{\bc_i\}_{i=1}^{n}$ for each node simultaneously using proximal update steps along with multiple local iterations before each communication round. Collaboration between workers is encouraged through a penalty term in the local objectives \eqref{qpfl} against a globally trained model $\bw$. Thus, compared to most recent works in federated learning which only aim to learn individual personalized models \TODO{CITE}, in addition to learning personalized models, QuPeL also learns a set of quantization vectors to compress each personalized model during for inference. Importantly, these quantization vectors for nodes $\{\bc_i\}_{i=1}^{n}$ can be different in length which allows QuPeL to learn models with different precision for each node based on memory constraints at deployment. Thus the model is personalized with respect to both the data distribution at the node (which address the data heterogeneity aspect of federated learning) and also the memory constraints of the node during inference (which address system heterogeneity of the participating devices).

\subsection{QuPeL: Quantized Personalized Learning}

\begin{algorithm}[H]
	\caption{QuPeL: Quantized Personalization Learning}
	{\bf Input:} Regularization parameters for quantization and personalization  $\lambda,\lambda_p $ respectively, synchronization gap \( \tau \).  For each worker $i$, initial full precision personalized model, initial quantization vectors (centers) and initial local model: $\bz_{i}^{{0}}=(\bx_{i}^{(0)},\bc_{i}^{(0)},\bw_{i}^{(0)})$. A penalty function enforcing quantization $R(\bx,\bc)$, \TODO{a soft quantization function $\widetilde{Q}_{\bc}(\bx)$}. Learning rates $\eta_1,\eta_2,\eta_3$.\\
	\vspace{-0.3cm}
	\begin{algorithmic}[1] \label{algo:personalized}
		\FOR{$t=0$ \textbf{to} $T-1$}
		\STATE \textbf{On Clients} $i=1$ \textbf{to} $n$ (in parallel) \textbf{do}:
		\IF{\TODO{$\tau$ does not divide $t$}}
		\STATE Compute $\bg_{i}^{t} := \nabla_{\bx_{i}^{t}} f_i(\bx_{i}^{t}) + \nabla_{\bx_{i}^{t}} f_i(\widetilde{Q}_{\bc_{i}^{t}}(\bx_{i}^{t})) $
		\STATE $\bx_{i}^{t+1}=\text{prox}_{\eta_1 \lambda R_{\bc_{i}^{t}}}(\bx_{i}^{t} - \eta_1 (\bg_{i}^{t} + \lambda_p(\bx_{i}^{t}-\bw_{i}^{t}))  )$\\
		\STATE Compute $\bh_i^{t} := \nabla_{\bc_{i}^{t}} f_i(\widetilde{Q}_{\bc_{i}^{t}}(\bx_{i}^{t+1})) $
		\STATE $\bc_{i}^{t+1}=\text{prox}_{\eta_2 \lambda R_{\bx_{i}^{t+1}}}(\bc_{i}^{t}-\eta_2 \bh_i^{t}  )$\\
		\STATE $\bw_{i}^{(t+1)} = %w_{i,t}-\eta_3 \nabla_{w_{t}} F_i(x_{i,t+1},c_{i,t+1},w_{i,t})=
		\bw_{i}^{t}-\eta_3 \lambda_p (\bx_{i}^{t+1}-\bw_{i}^{t}) $\\
		\ELSE
			\STATE Send $\bw_{i}^{t}$ to \textbf{Server}
			\STATE Receive $\bw^{t}$ from \textbf{Server} and set $\bw_i^{t+1} = \bw^{t}$
		\ENDIF
		\STATE \textbf{On Server:}
		\IF{\TODO{$\tau$ divides $t$}}
%		\STATE $\bw^{t+1} = \bw^{t}$
%		\ELSE
		\STATE Receive $\{\bw_i^{t}\}_{i=1}^n$ and compute $\bw^{t} := \frac{1}{n} \sum_{i=1}^n \bw_i^{t}$
		\STATE Broadcast $\bw^{t}$ to all \textbf{Clients}
		\ENDIF		
		\ENDFOR
		\STATE $\hat{\bx}_{i}^{T} = Q_{\bc_{i}^{T}}(\bx_{i}^{T})$ for all $i \in [n]$
	\end{algorithmic}
	{\bf Output:} Quantized personalized models $\hat{\bx}_i^{T}$ for $i \in [n]$
\end{algorithm}

We now formally discuss the update steps of QuPeL when run for $T$ iterations. Note that the local objective for each node $i \in [n]$ in \eqref{qpfl} can be split into two terms: the loss function $f_i(\bx_i) + f_i(\widetilde{Q}^{(i)}_{\bc_i}(\bx_i))+ \frac{\lambda_p}{2} \|\bx_i - \bw \|^2$ and the quantization loss term $\lambda R(\bx_i,\bc_i)$. To optimize over this objective, at each time step $t \in [T]$, node $i \in [n]$ maintains three parameters: model $\bx_i^{(t)}$, quantization vector $\bc_i^{(t)}$ and a copy of the global model $\bw_i^{(t)}$ (as we perform local iterations). At any step $t$ which is not a communication round (i.e. condition in line 2 is satisfied), the node first computes the gradient of the loss part of the objective w.r.t. the model $\bx_i^{(t)}$ and then takes a gradient step along with a proximal mapping using the quantization function $R$ (line 3-4) to form the updated parameter $\bx_i^{(t+1)}$. It then takes the gradient of the loss function w.r.t. the quantization vector $\bc_i^{(t)}$ and takes the update step for the centers along with a proximal step (line 5-6). Finally, the local copy of the global model is updated by taking a gradient step using gradient of the loss function w.r.t. $\bw_i^{(t)}$. The update steps in line 4 and line 6 ensure that the local personal model and the centers are simultaneously updated while being tied together by the quantization inducing term $R$ due to the proximal step. Furthermore, the local training of these parameters also incorporates knowledge from other nodes participating in the training through the parameter $w_i^{(t)}$. In the communication round (when $t$ is divisble by $\tau$), the nodes upload the local copies $\{\bw_i^{(t)}\}$ to the central server (\TODO{line}) which then performs an averaging step and communicates the updates global parameter to each node \TODO{line}. At the end of training, nodes learn a set of personalized models and centers, $\{\bx_i^{(T)}\}_{i=1}^{n}$ and $\{\bc_i^{(T)}\}_{i=1}^{n}$ respectively. Each node $i \in [n]$ then compresses the learned model $\bx_i^{(T)}$ to values in $\bc_i^{(T)}$  using the quantization mapping $Q^{(i)}$ (defined in \TODO{DEFINITION}), forming the compressed model $\hat{\bx}_i^{(T)}$ (line 14) which can be deployed in resource constrained environment for inference. 

\subsection{Theoretical results}

We now discuss the convergence rate for QuPeL for general convex objectives.\\
\textbf{Assumptions:}
Some of these are extensions of assumptions made in Section~\ref{subsec:main-1} to case of multiple workers:

{\sf (vi) } \textbf{Lower bound on local objective:} 
\begin{align*}
F_i(\bx,\bc,\bw)\geq 0\, , \forall i \in [n], \forall \bx\in \mathbb{R}^d, \bc \in \mathbb{R}^m, \bw \in \mathbb{R}^d
\end{align*}
{\sf (vii)} \textbf{Smoothness of \TODO{objectives}}: $f_i$ is $L_i$ smooth for $i \in [n]$. \\
{\sf (viii)}  \textbf{Bounded gradient}: There exists constant $G<\infty$ s.t.:
\begin{align*}
\Vert \nabla f_i \Vert_2 \leq G \, \quad \forall\bx \in \mathbb{R}^d, i\in [n]
\end{align*} 
{\sf (ix)} \textbf{Smoothness of soft quantizers:} For each node $i \in [n], $assumptions {\sf (iv)} hold for the soft quantization function $\tilde{Q}^{(i)}_{\bc}(\bx)$ with constants $L^{(i)}_{Q_1}$, $l^{(i)}_{Q_1}$, $L^{(i)}_{Q_2}$, $l^{(i)}_{Q_2}$ respectively. \\
{\sf (x)} \textbf{Bound on partial gradient of soft quantizers:} For each node $i \in [n]$, assumption {\sf (v)} holds for the soft quantization function $\tilde{Q}^{(i)}_{\bc}(\bx)$ with constants $G^{(i)}_{Q_1}$, $G^{(i)}_{Q_2}$. \\
{\sf (xi)} \TODO{\textbf{Bounded diversity:}}
At any $t \in [T]$, the variance of local gradients w.r.t. the global gradient is bounded:
\begin{align*}
& \Big\|\frac{1}{n} \sum_{j=1}^n \nabla_{\bw} F_j(\bx_{j}^{t},\bc_{j}^{t},\bw^{t} )-\nabla_{\bw} F_i(\bx_{i}^{t},\bc_{i}^{t},\bw) \Big\|^2 \leq \kappa_i,
\end{align*}
where $\text{Let } \nabla_{\bw^t} F(\{bx_{i}^{t}\}^n_i,\{\bc_{i}^{t}\}^n_i,\bw^{t}) = \frac{1}{n} \sum_{i=1}^n \nabla_{\bw^{t}} F_i(\bx_{i}^{t},\bc_{i}^{t},\bw^{t} )$. We also define $\kappa:=\frac{1}{n}\sum_{i=1}^n \kappa_i$


\begin{theorem} \label{thm:personalized}
	Let $\bG_{i}^{t} := [\nabla_{\bx_{i}^{t+1}} F_i(\bx_{i}^{t+1},\bc_{i}^{t},\bw^{t})]^T, \\ \nabla_{\bc_{i}^{t+1}} F_i(\bx_{i}^{t+1},\bc_{i}^{t+1},\bw^{t})^T, \nabla_{\bw^{t}} F_i(\bx_{i}^{t+1},\bc_{i}^{t+1},\bw^{t})^T]^T$ be the concatenated vector of gradients for any node $i \in [n]$. Consider running Algorithm \ref{algo:personalized} for $T$ iterations. Then for $\tau \leq \sqrt{T}$ and $\eta_3 = \frac{1}{4\lambda_p\sqrt{T}}$ \TODO{$\eta_1,\eta_2$?}, we have:
	
	%	\begin{align*}
	%	\frac{1}{T}\sum_{t=0}^{T-1}\frac{1}{n}\sum_{i=1}^{n} \Big\|G_{i,t}\Big\|^2 \leq& \frac{54(L^{(i)}_{max})^2\tau\kappa+108(L^{(i)}_{max})^2+288(L^{(i)}_{max})^2\lambda_p \Delta_F}{\sqrt{T}} + \frac{189\tau^2\kappa+\frac{3}{4}\tau^2\kappa^2}{T} + \frac{378\tau^2\kappa}{T^{\frac{3}{2}}}+ 216\kappa
	%	\end{align*}
	
	\begin{align*}
	\frac{1}{T}\sum_{t=0}^{T-1}\frac{1}{n}\sum_{i=1}^{n} \Big\|\bG_{i}^{t}\Big\|^2 \leq & \frac{\Lambda}{\sqrt{T}} + \frac{L_{max}^2\tau^2\kappa+\tau^2\kappa^2}{T}  \\  & \quad +\frac{L_{max}^2\tau^2\kappa}{T^{\frac{3}{2}}}+ L_{max}^2\kappa
	\end{align*}
	where $\Lambda = L_{max}^2\tau\kappa+L_{max}^2+L_{max}^2\lambda_p \Delta_F$ with $\Delta_F=\frac{\sum_{i=1}^{n}\left(F_i(\bx_{i}^{0},\bc_{i}^{0},\bw_{i}^{0})-F_i(\bx_{i}^{T},\bc_{i}^{T},\bw_{i}^{T})\right)}{n}$, and $L_{max} =\max\{\bigcup_{i=1}^n\{\lambda_p+L+GL^{(i)}_{Q_2}+G^{(i)}_{Q_2}Ll^{(i)}_{Q_2},GL^{(i)}_{Q_1}+G^{(i)}_{Q_1}Ll^{(i)}_{Q_1},1\}\}. $
\end{theorem}

In the above result $\Vert \bG_i \Vert_2^2$ refers to the sum of gradient norm of the local objective $F_i(\bx,\bc,\bw)$ w.r.t. to the parameters $\bx_i$, $\bc_i$ and $\bw_i$. Theorem \ref{thm:personalized} establishes a bound on the running time average of the norm of the gradients averaged across nodes. The bound shows convergence of this quantity to a constant dictated by $\kappa$, which is the gradient dissimilarity among clients, matching the rates \TODO{CITE}.

We provide a proof sketch for Theorem \ref{thm:personalized} in \TODO{REF} and provide a full proof in the \TODO{Appendix}

==> explore.tex <==
In the current state, the optimality result \eqref{eq:opt_result} still holds, while the result for constraint violation (and thus arguing that the proposed optimal solution also lies in the feasible set of the problem considered) is problematic. The problem in the analysis is the choice of $\blambda = \frac{\left[ \mathbb{E} \left[ \sum_{t=1}^{T} \bg(\bx^{(t)})  \right]  \right]^{+}}{\delta \eta T + \frac{1}{\eta}}$ (shown in red color in write-up). This at worse could be unbounded, contrary to Assumption {\bf A.3}. This also affects the bound on $\Vert \nabla_{\bx} \mathcal{L}_t(\bx,\blambda) \Vert$ given by $H$ which has thus been written in red in this write-up to emphasize this fact. \\
The bound on $\Vert \nabla_{\bx} \mathcal{L}_t(\bx,\blambda) \Vert$ is required to bound the quantization error $\Vert \be^{(t)} \Vert$ given in Lemma \ref{lem:e_t}. Having an unbounded $H$ (because of $\lambda$) will make the bound in Lemma \ref{lem:e_t} vacuous. \\
 Some potential fixes we can look at are:
\begin{itemize}
	\item Try to see if a different choice of value of $\blambda$ which makes it not unbounded can be made.
	\item Try to change the initial part of the analysis from \eqref{eq:proof_1} to \eqref{eq:proof_8} so as to introduce the quantization error term $\be^{(t)}$ later on. This might also require changing the update steps of the proposed algorithm. Note that to use the analysis in Lemma \ref{lem:e_t}, we would still require the norm of gradient of the Lagrangian to be bounded.
\end{itemize}

